The Kinematics and Dark Matter Fractions of TNG50 Galaxies at z=2 from an Observational Perspective

We contrast the gas kinematics and dark matter contents of $z=2$ star-forming galaxies (SFGs) from state-of-the-art cosmological simulations within the $\Lambda$CDM framework to observations. To this end, we create realistic mock observations of massive SFGs ($M_*>4\times10^{10} M_{\odot}$, SFR $>50~M_{\odot}$ yr$^{-1}$) from the TNG50 simulation of the IllustrisTNG suite, resembling near-infrared, adaptive-optics assisted integral-field observations from the ground. Using observational line fitting and modeling techniques, we analyse in detail the kinematics of seven TNG50 galaxies from five different projections per galaxy, and compare them to observations of twelve massive SFGs by Genzel et al. (2020). The simulated galaxies show clear signs of disc rotation but mostly exhibit more asymmetric rotation curves, partly due to large intrinsic radial and vertical velocity components. At identical inclination angle, their one-dimensional velocity profiles can vary along different lines of sight by up to $\Delta v=200$ km s$^{-1}$. From dynamical modelling we infer rotation speeds and velocity dispersions that are broadly consistent with observational results. We find low central dark matter fractions compatible with observations ($f_{\rm DM}^v(<R_e)=v_{\rm DM}^2(R_e)/v_{\rm circ}^2(R_e)\sim0.32\pm0.10$), however for disc effective radii $R_e$ that are mostly too small: at fixed $R_e$ the TNG50 dark matter fractions are too high by a factor of $\sim2$. We speculate that the differences in gas kinematics and dark matter content compared to the observations may be due to physical processes that are not resolved in sufficient detail with the numerical resolution available in current cosmological simulations.

==> macros.tex <==
%%%%%% General
\def\LCDM{$\Lambda\mbox{CDM}$}
\def\omm{\Omega_{\rm m}}
\def\oml{\Omega_{\Lambda}}
\def\omb{\Omega_{\rm b}}
\def\Ha{{\rm H\alpha}}
\def\Hb{{\rm H\beta}}
\def\tsf{t_{\rm SF}}
\def\AREPO{{\small AREPO}}
\def\GADGET{{\small GADGET}}
\def\GADGETTWO{{\small GADGET-2}}
\def\FOF{{\small FOF}}
\def\SUBFIND{{\small SUBFIND}}
\def\Illustris{{\it Illustris}}
\def\IllustrisDark{{\it Illustris-Dark}}
\def\SFR{{\rm SFR}}
\def\log{{\rm\thinspace log}}
\def\logten{{\rm\thinspace log_{10}}}

%%%%%% Control
\newcommand{\se}[1]{\S~(\ref{s:#1})}
\newcommand{\ifm}[1]{\relax\ifmmode#1\else$\mathsurround=0pt #1$\fi}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
% MNRAS
\newcommand{\equ}[1]{equation (\ref{e:#1})}
\newcommand{\equs}[1]{equations (\ref{e:#1})} % for historical reasons
\newcommand{\eqs}[2]{equations (\ref{e:#1}) and (\ref{e:#2})} % use this
\newcommand{\Equ}[1]{Equation (\ref{e:#1})}
\newcommand{\Equs}[1]{Equations (\ref{e:#1})} % for historical reasons
\newcommand{\Eqs}[2]{Equations (\ref{e:#1}) and (\ref{e:#2})} % use this
\newcommand{\Fig}[1]{Fig.~\ref{f:#1}}
\newcommand{\Figs}[2]{Figs.~\ref{f:#1} and \ref{f:#2}}
% ApJ
%\newcommand{\Fig}[1]{Figure (\ref{f:#1})}
%\newcommand{\Figs}[2]{Figures (\ref{f:#1}) and (\ref{f:#2})}

%%%%%% Colors
\newcommand{\sgr}[1]{\textcolor{red}{#1}}
\newcommand{\sgb}[1]{\textcolor{blue}{#1}}
\newcommand{\sgg}[1]{\textcolor{green}{[#1]}}
\newcommand{\sggg}[1]{\textcolor{green}{[]}}
\newcommand{\sgrcm}[1]{\textcolor{red}{[SG: #1]}}

%%%%%% Units
\def\dex{{\rm\thinspace dex}}
\def\cm{{\rm\thinspace cm}}
\def\km{{\rm\thinspace km}}
\def\m{{\rm\thinspace m}}
\def\micron{{\rm\thinspace \mu m}}
\def\AAA{{\rm\thinspace \AA}}
\def\pc{{\rm\thinspace pc}}
\def\kpc{{\rm\thinspace kpc}}
\def\Mpc{{\rm\thinspace Mpc}}
\def\Mpccb{\,{\rm Mpc}^{3}}
\newcommand{\hMpc}{\,\ifm{h^{-1}}{\rm Mpc}}
\newcommand{\hkpc}{\,\ifm{h^{-1}}{\rm kpc}}
\def\kms{{\rm\thinspace km\thinspace s}^{-1}}
\def\pcmsq{{\rm\thinspace cm}^{-2}}
\def\pcmcb{{\rm\thinspace cm}^{-3}}
\def\pMpccb{\,{\rm Mpc}^{-3}}
\def\eV{{\rm\thinspace eV}}  
\def\keV{{\rm\thinspace keV}}
\def\GeV{{\rm\thinspace GeV}}
\def\erg{{\rm\thinspace erg}}
\def\ergs{{\rm\thinspace erg s}^{-1}}
\def\g{{\rm\thinspace g}} 
\def\kg{{\rm\thinspace kg}}
\def\Lsun{\hbox{$\rm\thinspace L_{\odot}$}}
\def\Msun{\hbox{$\rm\thinspace M_{\odot}$}}
\def\Zsun{\hbox{$\rm\thinspace Z_{\odot}$}}
\def\s{{\rm\thinspace s}}       
\def\yr{{\rm\thinspace yr}}
\def\Myr{{\rm\thinspace Myr}}
\def\Gyr{{\rm\thinspace Gyr}}
\def\Gyrinv{{\Gyr^{-1}}}
\def\Msunyr{\Msun\yr^{-1}}
\def\Msunpc2{{\Msun\pc}^{-2}}
\def\Msunyrkpc2{{\Msun\yr^{-1}\kpc}^{-2}}
\def\arcsec{{\rm\thinspace arcsec}}
\def\magarcsec2{{\rm\thinspace mag\thinspace arcsec}^{-2}}
\def\CPUh{{\rm\thinspace CPU-hours}}
\def\kB{{\rm\thinspace kB}}
\def\MB{{\rm\thinspace MB}}
\def\GB{{\rm\thinspace GB}}
\def\TB{{\rm\thinspace TB}}

